Learning Set Functions with Implicit Differentiation

Ou et al. (2022) introduce the problem of learning set functions from data generated by a so-called optimal subset oracle. Their approach approximates the underlying utility function with an energy-based model, whose parameters are estimated via mean-field variational inference. Ou et al. (2022) show this reduces to fixed point iterations; however, as the number of iterations increases, automatic differentiation quickly becomes computationally prohibitive due to the size of the Jacobians that are stacked during backpropagation. We address this challenge with implicit differentiation and examine the convergence conditions for the fixed-point iterations. We empirically demonstrate the efficiency of our method on synthetic and real-world subset selection applications including product recommendation, set anomaly detection and compound selection tasks.

==> tex/8_reproducibility.tex <==
This paper:
\begin{itemize}
    \item \textit{Includes a conceptual outline and/or pseudocode description of AI methods introduced:} \textbf{Yes.}
    
    We include the conceptual outlines and the pseudocodes for the competitor algorithm and our proposed algorithm in Sections~\ref{sec: setup}~\&~\ref{sec:contributions}.

    \item \textit{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results:} \textbf{Yes.}

    \item \textit{Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper:} \textbf{Yes.}

    \item \textit{Does this paper make theoretical contributions?: } \textbf{Yes.}

    \textit{If yes, }%please complete the list below.
    \begin{itemize}
        \item \textit{All assumptions and restrictions are stated clearly and formally:} \textbf{Yes.} 

        Please see Asm.~\ref{asm:bound}.

        \item \textit{All novel claims are stated formally (e.g., in theorem statements):} \textbf{Yes.}

        Please see Theorems~\ref{thm:banach}~\&~\ref{thm:implicit_result}.

        \item \textit{Proofs of all novel claims are included:} \textbf{Yes.}

        Please see Appendices~\ref{app:convergence}~\&~\ref{app:AandB}.

        \item \textit{Proof sketches or intuitions are given for complex and/or novel results:} \textbf{Yes.}

        We motivate the reader for the necessity of our novel results in Sections~\ref{sec:challenges}~\&~\ref{sec:contributions}. Moreover, in Sec.~\ref{sec:contributions} we state that the proofs of our theorems rely on the Banach fixed-point and implicit function theorems.

        \item \textit{Appropriate citations to theoretical tools used are given:} \textbf{Yes.}

        \item \textit{All theoretical claims are demonstrated empirically to hold:} \textbf{Yes.}

        \item \textit{All experimental code used to eliminate or disprove claims is included:} \textbf{N/A.}

        \item \textit{Does this paper rely on one or more datasets?} \textbf{Yes.}

        \textit{If yes, }
        \begin{itemize}
            \item \textit{A motivation is given for why the experiments are conducted on the selected datasets: } \textbf{Yes.}

            \item \textit{All novel datasets introduced in this paper are included in a data appendix:} \textbf{N/A.}

            \item \textit{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes:} \textbf{N/A.}

            \item \textit{All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations:} \textbf{Yes.}

            \item \textit{All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available:} \textbf{Yes.}

            \item \textit{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing:} \textbf{N/A.}

            \item \textit{Does this paper include computational experiments?} \textbf{Yes.}

            \textit{If yes,}
            \begin{itemize}
                \item \textit{Any code required for pre-processing data is included in the appendix:} \textbf{Yes.}

                All source code, including any code for pre-processing data, is included in the supplementary material.

                \item \textit{All source code required for conducting and analyzing the experiments is included in a code appendix:} \textbf{Yes.}

                \item \textit{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes:} \textbf{Yes.}

                \item \textit{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from:} \textbf{Yes.}

                \item \textit{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results:} \textbf{Yes.}

                \item \textit{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks:} \textbf{Yes.}

                \item \textit{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics:} \textbf{Yes.}

                \item \textit{This paper states the number of algorithm runs used to compute each reported result:} 

                \item \textit{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information:} \textbf{Yes.}

                \item \textit{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank):} \textbf{No.} 

                \item \textit{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments:} \textbf{Yes.}

                \item \textit{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting:} \textbf{Yes.}
            \end{itemize}

        \end{itemize}
    \end{itemize}
\end{itemize}
